A Complexity-Based Hierarchy for Multiprocessor Synchronization

For many years, Herlihy's elegant computability based Consensus Hierarchy has been our best explanation of the relative power of various types of multiprocessor synchronization objects when used in deterministic algorithms. However, key to this hierarchy is treating synchronization instructions as distinct objects, an approach that is far from the real-world, where multiprocessor programs apply synchronization instructions to collections of arbitrary memory locations. We were surprised to realize that, when considering instructions applied to memory locations, the computability based hierarchy collapses. This leaves open the question of how to better capture the power of various synchronization instructions. In this paper, we provide an approach to answering this question. We present a hierarchy of synchronization instructions, classified by their space complexity in solving obstruction-free consensus. Our hierarchy provides a classification of combinations of known instructions that seems to fit with our intuition of how useful some are in practice, while questioning the effectiveness of others. We prove an essentially tight characterization of the power of buffered read and write instructions.Interestingly, we show a similar result for multi-location atomic assignments.

==> header.tex <==
\usepackage{amsthm} % provides an enhanced version of LaTeX's \newtheorem 
%\usepackage[papersize={8.5in,11in},margin=1in]{geometry}
%%command for defining theorem-like environments
%\usepackage{times}
\usepackage{comment}
%\usepackage{fancyhdr} % extensive control of page headers and footers in 
%%LaTeX2e
\usepackage{tabularx}
\usepackage{adjustbox}
\usepackage{graphicx}
%  \pagestyle{plain}
%%\usepackage[camera]{dtrt}
%\usepackage{color} % color control for LaTeX documents
%\usepackage{changepage}
%%\usepackage{algorithm} % floating environment for algorithms
%%\usepackage{algorithmic} % pseudocode support
%\usepackage[nofillcomment,linesnumbered,noend,noresetcount,noline]{algorithm2e}
%%\usepackage[boxruled,linesnumbered,nofillcomment,noend,noline]{algorithm2e}
%%\widowpenalty=0
%%\clubpenalty=10000
%%\interfootnotelinepenalty=0
%\newcommand{\parhead}[1]{\medskip \noindent {\bfseries\boldmath\ignorespaces 
%#1.}\hskip 0.9em plus 0.3em minus 0.3em}
%%\setlength{\footskip}{1\baselineskip}
%\AtBeginDocument{%
% \abovedisplayskip=2pt plus 1pt minus 1pt
% \abovedisplayshortskip=0pt plus 1pt
% \belowdisplayskip=2pt plus 1pt minus 1pt
% \belowdisplayshortskip=0pt plus 1pt
%}
%\usepackage{array}
%\setlength\extrarowheight{2pt}
%
%\usepackage[noindentafter]{titlesec}
%\titlespacing{\paragraph}{%
%  0pt}{%              left margin
%  0.1\baselineskip}{% space before (vertical)
%  1em}%               space after (horizontal)
%\titlespacing\section{0pt}{8pt plus 1pt minus 1pt}{2pt plus 1pt minus 1pt}
%\titlespacing\subsection{0pt}{8pt plus 1pt minus 1pt}{2pt plus 1pt minus 1pt}
%\titlespacing\subsubsection{0pt}{8pt plus 1pt minus 1pt}{2pt plus 1pt minus 
%1pt}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% PACKAGES and SETTINGS
%%\usepackage{anysize} % a simple package to set up document margins
%%\marginsize{1in}{1in}{1in}{1in}
% %\pagestyle{headings}
%%\usepackage{amsmath} % enhances the typeset appearance of mathematical 
%%%formulas
%%\usepackage{amssymb} % subset of amsfonts that defines the full set of symbol 
%%%names for two fonts of extra symbols included in amsfonts
%\usepackage{graphicx} % enhanced support for graphics
%\usepackage{complexity} % computational complexity class names
%%\usepackage[numbers]{natbib} % flexible bibliography support
%%\usepackage{colortbl} % add color to LaTeX tables
%%\usepackage[colorinlistoftodos,textwidth=4cm]{todonotes} % marking things to 
%%%do in a LaTeX document
%%\usepackage{setspace} % set space between lines
% %\usepackage{minitoc} % produce a table of contents for each chapter, part or 
%%%section
%\usepackage{enumitem} % control layout of itemize, enumerate, description
%%\usepackage{floatrow} % modifying the layout of floats
%\usepackage{shorttoc} % table of contents with different depths
%\usepackage{array} % extending the array and tabular environments
%%\usepackage{tikz} % create PostScript and PDF graphics in TeX
%%  \usetikzlibrary{shapes,arrows,topaths}
%%\usepackage{float}
%%\usepackage{subfig}
%%\usepackage{tabularx} % tabulars with adjustable-width columns
%%\usepackage{stmaryrd}
%%\usepackage{cancel}
%%\usepackage{cases}
%%\usepackage[us]{datetime}
%%\usepackage{mathrsfs}
%\usepackage{float}
%%\usepackage[maxfloats=100]{morefloats}
%\usepackage{pdfsync}
%\usepackage{verbatim}
%\newcommand{\dtlinkcolor}{{0.8 0.8 1}} % link color, RGB
%\usepackage[hyperindex=true,pdfpagemode=UseOutlines,bookmarksnumbered=true,bookmarksopen=true,bookmarksopenlevel=2,pdfstartview=FitH,pdfborder={0
% 0 
%1},linkbordercolor=\dtlinkcolor,citebordercolor=\dtlinkcolor,urlbordercolor=\dtlinkcolor,pagebordercolor=\dtlinkcolor]{hyperref}
%\hypersetup{pageanchor=false}

%Adding backreferencing
\usepackage[colorlinks]{hyperref}
\hypersetup{linkcolor=red,filecolor=red,citecolor=red,urlcolor=red}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% THEOREMS

%\newtheoremstyle{slplain}% name
%  {.4\baselineskip\@plus.1\baselineskip\@minus.1\baselineskip}% Space above
%  {.3\baselineskip\@plus.1\baselineskip\@minus.1\baselineskip}% Space below
%  {\itshape}% Body font
%  {}%Indent amount (empty = no indent, \parindent = para indent)
%  {\bfseries}%  Thm head font
%  {.}%       Punctuation after thm head
%  { }%      Space after thm head: " " = normal interword space;
%        %       \newline = linebreak
%  {}%       Thm head spec
%\theoremstyle{slplain} % italics
%
%%\newtheorem{ctheorem}{Theorem}
\newtheorem*{definition*}{Definition}
\newtheorem*{theorem*}{Theorem}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{fact}[theorem]{Fact}
%\newenvironment{ptheorem}[2][Theorem]{\begin{trivlist}
%\item[\hskip \labelsep {\bfseries #1}\hskip \labelsep {\bfseries \emph{#2}}]}{\end{trivlist}}


%\makeatletter
%\newtheorem*{rep@theorem}{\rep@title}
%\newcommand{\newreptheorem}[2]{%
%\newenvironment{rep#1}[1]{%
% \def\rep@title{#2 \ref{##1}}%
% \begin{rep@theorem}}%
% {\end{rep@theorem}}}
%\makeatother
%
%\newreptheorem{theorem}{Theorem}
%\newreptheorem{lemma}{Lemma}
%\newreptheorem{claim}{Claim}
%\newreptheorem{corollary}{Corollary}
%
%
%\theoremstyle{definition}
%\newtheorem{construction}[theorem]{Construction}
%\newtheorem{conjecture}{Conjecture}[section]
%\newtheorem{example}[theorem]{Example}
%\newtheorem{remark}[theorem]{Remark}
%
%\theoremstyle{remark}
%\newtheorem*{note}{Note}
%\newtheorem{case}{Case}

%\numberwithin{equation}{section}

%\newtheoremstyle{etplain}% name
%  {.0\baselineskip\@plus.1\baselineskip\@minus.1\baselineskip}% Space above
%  {.0\baselineskip\@plus.1\baselineskip\@minus.1\baselineskip}% Space below
%  {\itshape}% Body font
%  {}%Indent amount (empty = no indent, \parindent = para indent)
%  {\bfseries}%  Thm head font
%  {.}%       Punctuation after thm head
%  { }%      Space after thm head: " " = normal interword space;
%        %       \newline = linebreak
%  {}%       Thm head spec
%\theoremstyle{etplain} % italics
%\newtheorem{sstheorem}{Theorem}
%\usepackage[style=0,skipabove=3pt,skipbelow=2pt,innertopmargin=2pt,innerbottommargin=2pt]{mdframed}
%\newenvironment{stheorem}
%  {\begin{mdframed}\begin{sstheorem}}
%  {\end{sstheorem}\end{mdframed}}
%\newtheorem{innercustomthm}{Theorem}
%\newenvironment{ctheorem}[1]
%  {\begin{mdframed}\renewcommand\theinnercustomthm{#1}\innercustomthm}
%  {\endinnercustomthm\end{mdframed}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% REFERNCE MACROS

\newcommand{\idlow}[1]{\mathord{\mathcode`\-="702D\it #1\mathcode`\-="2200}}
\newcommand{\id}[1]{\ensuremath{\idlow{#1}}}
\newcommand{\litlow}[1]{\mathord{\mathcode`\-="702D\sf #1\mathcode`\-="2200}}
\newcommand{\lit}[1]{\ensuremath{\litlow{#1}}}

\newcommand{\rl}{\lit{read\_last}()}
\newcommand{\rn}{\lit{read}()}
\newcommand{\sap}[1]{\lit{store\_and\_read}(#1)}

\newcommand{\namedref}[2]{\hyperref[#2]{#1~\ref*{#2}}}

\newcommand{\chapterref}[1]{\namedref{Chapter}{#1}}
\newcommand{\sectionref}[1]{\namedref{Section}{#1}}
\newcommand{\appendixref}[1]{\namedref{Appendix}{#1}}
\newcommand{\theoremref}[1]{\namedref{Theorem}{#1}}
\newcommand{\factref}[1]{\namedref{Fact}{#1}}
\newcommand{\observationref}[1]{\namedref{Observation}{#1}}
\newcommand{\remarkref}[1]{\namedref{Remark}{#1}}
\newcommand{\definitionref}[1]{\namedref{Definition}{#1}}
\newcommand{\figureref}[1]{\namedref{Figure}{#1}}
\newcommand{\figurerefb}[2]{\hyperref[#1]{Figure~\ref*{#1}#2}}
\newcommand{\tableref}[1]{\namedref{Table}{#1}}
\newcommand{\lemmaref}[1]{\namedref{Lemma}{#1}}
\newcommand{\claimref}[1]{\namedref{Claim}{#1}}
\newcommand{\propositionref}[1]{\namedref{Proposition}{#1}}
\newcommand{\corollaryref}[1]{\namedref{Corollary}{#1}}
\newcommand{\constructionref}[1]{\namedref{Construction}{#1}}
\newcommand{\itemref}[1]{\namedref{Item}{#1}}
\newcommand{\propertyref}[1]{\namedref{Property}{#1}}
\newcommand{\protocolref}[1]{\namedref{Protocol}{#1}}
\newcommand{\algorithmref}[1]{\namedref{Algorithm}{#1}}
\newcommand{\assumptionref}[1]{\namedref{Assumption}{#1}}
\newcommand{\stepref}[1]{\namedref{Step}{#1}}
\newcommand{\paramref}[1]{\namedref{Parameter}{#1}}
\newcommand{\footnoteref}[1]{\namedref{Footnote}{#1}}
\newcommand{\equationref}[1]{\hyperref[#1]{(\ref*{#1})}}
\renewcommand{\eqref}{\equationref}
%\newcommand{\equationref}[1]{\namedref{Equation}{#1}}
\newcommand{\exampleref}[1]{\namedref{Example}{#1}}
\newcommand{\lineref}[1]{\namedref{Line}{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% MACROS %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% TODO macro
%\newcommand{\TODO}[1]{\todo[inline,color=green!20]{#1}\vspace{1mm}}
\usepackage[textsize=tiny]{todonotes}
\newcommand{\jtodo}[1]{\todo[color=blue!20]{#1}}
\newcommand{\rtodo}[1]{\todo[color=red!20]{#1}}
\newcommand{\jimmy}[1]{$\ll$\textsf{\color{red} Jimmy: #1}$\gg$}
\newcommand{\rati}[1]{$\ll$\textsf{\color{red} Rati: #1}$\gg$}


% DEBUG macro
\newcommand{\DEBUG}[1]{}

% arg max
\newcommand{\argmax}{\operatornamewithlimits{arg\,max}}
\newcommand{\argmin}{\operatornamewithlimits{arg\,min}}

% defeq
\newcommand{\defeq}{\stackrel{\mathrm{\scriptscriptstyle def}}{=}}
\newcommand{\defem}[1]{\textsf{#1}}

% Buffered instructions
\newcommand{\ellbw}{\ensuremath{\id{\ell-buffer-write}}}
\newcommand{\ellbr}{\ensuremath{\id{\ell-buffer-read}}}

%\newenvironment{newitemize}{%
%\begin{list}{$\bullet$}{\labelwidth=18pt%
%\labelsep=5pt \leftmargin=23pt \topsep=1pt%
%%\setlength{\listparindent}{\saveparindent}%
%\setlength{\listparindent}{0pt}%
%\setlength{\parsep}{\parskip}%
%\setlength{\itemsep}{3pt}}}{\end{list}}
%
%\newenvironment{newcenter}{%
%\begin{center}%
%\vspace{-5pt}%
%\setlength{\parskip}{0pt}}{\end{center}\vspace{-5pt}}


%\renewcommand{\hat}{\widehat}
%\renewcommand{\tilde}{\widetilde}
\renewcommand{\setminus}{-}
\renewcommand{\emptyset}{\varnothing}
\newcommand{\veps}{\varepsilon}
\newcommand{\vol}{\mathrm{vol}}
\renewcommand{\ln}{\log}  %Zeyuan: I'm happy to define it the other way around as well ;) Just to make sure on the consistency
\newcommand{\bR}{\mathbb{R}}
\newcommand{\EX}{\operatornamewithlimits{\mathbb{E}}}
\newcommand{\cA}{\mathcal{A}}

%\renewcommand{\algorithmicrequire}{\textbf{Input:}}
%\renewcommand{\algorithmicensure}{\textbf{Output:}}

%\def\bqed{\hfill$\blacksquare$}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

